Optimized Feature Space Learning for Generating Efficient Binary Codes for Image Retrieval

In this paper we propose an approach for learning low dimensional optimized feature space with minimum intra-class variance and maximum inter-class variance. We address the problem of high-dimensionality of feature vectors extracted from neural networks by taking care of the global statistics of feature space. Classical approach of Linear Discriminant Analysis (LDA) is generally used for generating an optimized low dimensional feature space for single-labeled images. Since, image retrieval involves both multi-labeled and single-labeled images, we utilize the equivalence between LDA and Canonical Correlation Analysis (CCA) to generate an optimized feature space for single-labeled images and use CCA to generate an optimized feature space for multi-labeled images. Our approach correlates the projections of feature vectors with label vectors in our CCA based network architecture. The neural network minimize a loss function which maximizes the correlation coefficients. We binarize our generated feature vectors with the popular Iterative Quantization (ITQ) approach and also propose an ensemble network to generate binary codes of desired bit length for image retrieval. Our measurement of mean average precision shows competitive results on other state-of-the-art single-labeled and multi-labeled image retrieval datasets.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> abbreviations.tex <==
% !TEX root = thesis.tex

%-----------------------------------------------------------------------------------
%  Abbreviations
%-----------------------------------------------------------------------------------

% Abbreviations in text, general
\ifnum\varDraft = 1
  % here, some work is required - todo item
  \newcommand*{\todo}[1]{{\fbox{\small\sl To do: #1}}}
  % missing reference
  \newcommand*{\uref}{{?.?.?}}
\fi
% separate file containing all common definitions and packages that are useful for setting formulas etc.
% so they will be consistent if they are included from MetaPost, Matplotlib, etc.
% \usepackage{xfrac}
% \usepackage{trsym}
% 
% \DeclareMathOperator{\rect}{rect}
% \DeclareMathOperator{\si}{si}
% \DeclareMathOperator{\Si}{Si}
% \DeclareMathOperator{\lb}{lb}
% \DeclareMathOperator{\erfc}{erfc}
% \DeclareMathOperator{\sinc}{sinc}
% \DeclareMathOperator{\sgn}{sgn}
% \DeclareMathOperator{\pdf}{p}
% \DeclareMathOperator{\prob}{P}
% \DeclareMathOperator*{\med}{med}
% \DeclareMathOperator{\expect}{E}
% 
% % imaginary and real part
% \renewcommand{\Im}{\operatorname{Im}}
% \renewcommand{\Re}{\operatorname{Re}}
% 
% % integral delta
\newcommand{\dd}{\;\mathrm{d}}
% 
% % zero and unit matrix
\newcommand{\0}{\mathbf{0}}
\newcommand{\1}{\mathbf{1}}
% 
% % fourier transform F
% \newcommand{\FT}{\mathcal{F}}
% \newcommand{\IFT}{\mathcal{F}^{-1}}
% 
% % transpose
\newcommand{\T}{\mathrm{T}}
% % complex unit
% \newcommand{\J}{\jmath}
% 
% % put an exponent on the left side of a quantity
% \newcommand{\leftexp}[2]{{\vphantom{#2}}^{#1}{#2}}
% 
% % magnitude
% \newcommand{\abs}[1]{\left\lvert#1\right\rvert}
% % norm
% \newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% 
% % z-transform bone symbols
% \newcommand{\zth}{\stackrel{\mathrm{Z}}{\TransformHoriz}}
% \newcommand{\izth}{\stackrel{\mathrm{Z}}{\InversTransformHoriz}}
% \newcommand{\ztv}{\TransformVert{}\mathrm{Z}}
% \newcommand{\iztv}{\InversTransformVert{}\mathrm{Z}}
% 
% % fourier transform bone symbols
% \newcommand{\fth}{\stackrel{\mathrm{F}}{\TransformHoriz}}
% \newcommand{\ifth}{\stackrel{\mathrm{F}}{\InversTransformHoriz}}
% \newcommand{\ftv}{\TransformVert{}\mathrm{F}}
% \newcommand{\iftv}{\InversTransformVert{}\mathrm{F}}
% 
% % number sets
% \newcommand{\setN}{\mathbb{N}}
\newcommand{\setR}{\mathbb{R}}
% \newcommand{\setC}{\mathbb{C}}
% \newcommand{\setZ}{\mathbb{Z}}
% 
% % use this to denote vectors and matrices (makes the symbol bold)
\renewcommand{\vec}[1]{{\boldsymbol{#1}}}
\newcommand{\mat}[1]{\boldsymbol{#1}}
% 
% % use this to reference an element of a vector or matrix
% \newcommand{\vecel}[2]{#1_{#2}}
% \newcommand{\matel}[2]{#1_{#2}}


==> abin.tex <==


\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,positioning,fit,petri, decorations.pathreplacing,shadows,calc}




%
%

%

%



%\documentclass[tikz,border=3.14pt]{standalone}
\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}



	

\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{
code={
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-right) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;

\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
 
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;

}
}}



% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}

\begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
font=\sffamily\small,scale=2]



\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.4,-\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 1}}] (\X - 0.2 ,0.9,0) -- (\X - 0.2, {2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,0.4) (hl) {Anchor};
}


%%% For the input 1


\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.5,-4*\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 2}}] (\X - 0.5 ,-1.5,0) -- (\X - 0.5, -{2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,-2.4) (hl) {Negative};
}
%%% For the input 2





\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X  - 0,-4*\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={CONV}}] (\X  ,-1.5,0) -- (\X  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.45,1.65) (hl) {};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1 ,-4*\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.35,1.45) (hl) {};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X + 0.2 ,-4*\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (3.35,1.25) (hl) { };
\node at (4.35,-2.15) (hl) {};
\node at (4.57, 0.90) (PU1){\textcolor{gray}{.}};
\node at (4.32,-0.48) (PD1){\textcolor{gray}{.}};
\node at (4.57,-0.58) (PU2){\textcolor{gray}{.}};
\node at (4.32,-2.00) (PD2){\textcolor{gray}{.}};




}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X ,-\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;


%\path[black,decorate,decoration={text effects along path,text={ conv}}] (\X + .05 ,0.5,0) -- (\X + .05 , -{2 + (-\Y)/2  - 2} ,0);
\node at (4.35,1.05) (hl) { };
\node at (3.25,-2.60) (hl) {};

}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1,-\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.15,-3.00) (hl) {};
}

%For the blocks 1


%For blocks below%


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.2,-\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.25,-3.35) (hl) {};
\node[diamond,aspect=3,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (GG1) at (0.72, 0.8) {};
\node[diamond,aspect=3,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (GG2) at (0.65, -1.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (F1) at (1.45, 0.8) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (F2) at (1.45, -1.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=2.5pt] (S1) at (2.42, 0.7) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=2.5pt] (S2) at (2.42, -1.45) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=2pt] (T1) at (3.5, 0.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=2pt] (T2) at (3.5, -1.3) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=1.5pt] (FF1) at (4.5, 0.5) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=1.5pt] (FF2) at (4.5, -1.1) {};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (GG1.east) -- (F1.east);
\draw[gray,dashed] (GG1.west) -- (F1.west);
\draw[gray,dashed] (GG1.north) -- (F1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (GG2.east) -- (F2.east);
\draw[gray,dashed] (GG2.west) -- (F2.west);
\draw[gray,dashed] (GG2.north) -- (F2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (F1.east) -- (S1.east);
\draw[gray,dashed] (F1.west) -- (S1.west);
\draw[gray,dashed] (F1.north) -- (S1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (F2.east) -- (S2.east);
\draw[gray,dashed] (F2.west) -- (S2.west);
\draw[gray,dashed] (F2.north) -- (S2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (S1.east) -- (T1.east);
\draw[gray,dashed] (S1.west) -- (T1.west);
\draw[gray,dashed] (S1.north) -- (T1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (S2.east) -- (T2.east);
\draw[gray,dashed] (S2.west) -- (T2.west);
\draw[gray,dashed] (S2.north) -- (T2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[gray,dashed] (T1.east) -- (FF1.east);
\draw[gray,dashed] (T1.west) -- (FF1.west);
\draw[gray,dashed] (T1.north) -- (FF1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (T2.east) -- (FF2.east);
\draw[gray,dashed] (T2.west) -- (FF2.west);
\draw[gray,dashed] (T2.north) -- (FF2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


}




%
%\node[draw,single arrow, orange,fill=orange!30] at (8,0.5,0) {GAP};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[circle,draw,blue,fill=blue!30] (A1) at (5,1,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,0.8,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\node[rectangle,draw,black,fill=orange!30]  (KL) at (7,-0.4,0) {KL Distance};
\node[rectangle,draw,black,fill=orange!30]  (Loss) at (8,-0.4,0) {LDA Loss};
\draw[-latex] (KL) -- (Loss);
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer){};
\node[above of=A1, node distance=0.5cm] (hl) {512};
\node[above of=B2, node distance=1.2cm] (hl) {9};
\draw[gray,dashed] (PD1) -- (A3);
\draw[gray,dashed] (PU1) -- (A1);
\end{scope}

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);

\node[circle,draw,blue,fill=blue!30] (A1) at (5,-0.7,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,-0.9,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer) {};
\node[above of=A1, node distance=0.5cm] (hl) {512};
\node[above of=B2, node distance=1.2cm] (hl) {9};
\draw[gray,dashed] (PD2) -- (A3);
\draw[gray,dashed] (PU2) -- (A1);
\end{scope}


\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);







\end{tikzpicture}







% 
% \def\layersep{2.5cm}
% [shorten >=1pt,->,draw=black!50, node distance=\layersep]
%     \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%     \tikzstyle{neuron}=[circle,fill=black!25,minimum size=10pt,inner sep=0pt]
%     \tikzstyle{square-out}=[square,fill=black!25,minimum size=20pt,inner sep=0pt]
%     \tikzstyle{input neuron}=[neuron, fill=green!50];
%     \tikzstyle{output neuron}=[square-out, fill=red!50];
%     \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%     \tikzstyle{annot} = [text width=4em, text centered]
% 
%     % Draw the input layer nodes
%     \foreach \name / \y in {1,...,10}
%     % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%         \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};
% 
%     % Draw the hidden layer nodes
%     \foreach \name / \y in {1,...,3}
%         \path[yshift=0.5cm]
%             node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};
% 
%     % Draw the output layer node
%     \node[output neuron,pin={[pin edge={->}]right:LDA Loss} , right of=H-2] (O) {KL-distance};
% 
%     % Connect every node in the input layer with every node in the
%     % hidden layer.
%     \foreach \source in {1,...,10}
%         \foreach \dest in {1,...,3}
%             \path (I-\source) edge (H-\dest);
% 
%     % Connect every node in the hidden layer with the output layer
%     \foreach \source in {1,...,3}
%         \path (H-\source) edge (O) ;
% 
%     % Annotate the layers
%     \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
%     \node[annot,left of=hl] {Input layer};
%     \node[annot,right of=hl] {LDA projection};
% \end{tikzpicture}


==> abin_final.tex <==


\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,positioning,fit,petri, decorations.pathreplacing,shadows,calc}




%
%

%

%



%\documentclass[tikz,border=3.14pt]{standalone}
\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}



	

\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{
code={
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-right) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;

\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
 
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;

}
}}



% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}

\begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
font=\sffamily\small,scale=2]



\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.4,-\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 1}}] (\X - 0.2 ,0.9,0) -- (\X - 0.2, {2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,0.4) (hl) {Img 1};
}


%%% For the input 1


\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.5,-4*\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 2}}] (\X - 0.5 ,-1.5,0) -- (\X - 0.5, -{2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,-2.4) (hl) {Img 2};
}
%%% For the input 2





\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X  - 0,-4*\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={CONV}}] (\X  ,-1.5,0) -- (\X  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.45,1.65) (hl) {};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1 ,-4*\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.35,1.45) (hl) {};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X + 0.2 ,-4*\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (3.35,1.25) (hl) { };
\node at (4.35,-2.15) (hl) {};
\node at (4.57, 0.90) (PU1){\textcolor{gray}{.}};
\node at (4.32,-0.48) (PD1){\textcolor{gray}{.}};
\node at (4.57,-0.58) (PU2){\textcolor{gray}{.}};
\node at (4.32,-2.00) (PD2){\textcolor{gray}{.}};




}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X ,-\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;


%\path[black,decorate,decoration={text effects along path,text={ conv}}] (\X + .05 ,0.5,0) -- (\X + .05 , -{2 + (-\Y)/2  - 2} ,0);
\node at (4.35,1.05) (hl) { };
\node at (3.25,-2.60) (hl) {};

}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1,-\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.15,-3.00) (hl) {};
}

%For the blocks 1


%For blocks below%


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.2,-\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.25,-3.35) (hl) {};
\node[diamond,aspect=3,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (GG1) at (0.72, 0.8) {};
\node[diamond,aspect=3,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (GG2) at (0.65, -1.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (F1) at (1.45, 0.8) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=3pt] (F2) at (1.45, -1.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=2.5pt] (S1) at (2.42, 0.7) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=2.5pt] (S2) at (2.42, -1.45) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=2pt] (T1) at (3.5, 0.6) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=2pt] (T2) at (3.5, -1.3) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,   inner sep=1.5pt] (FF1) at (4.5, 0.5) {};
\node[diamond,aspect=2.5,rotate=70, dashed, draw=black, fill=none,  fill opacity=0.1,  inner sep=1.5pt] (FF2) at (4.5, -1.1) {};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (GG1.east) -- (F1.east);
\draw[gray,dashed] (GG1.west) -- (F1.west);
\draw[gray,dashed] (GG1.north) -- (F1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (GG2.east) -- (F2.east);
\draw[gray,dashed] (GG2.west) -- (F2.west);
\draw[gray,dashed] (GG2.north) -- (F2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (F1.east) -- (S1.east);
\draw[gray,dashed] (F1.west) -- (S1.west);
\draw[gray,dashed] (F1.north) -- (S1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (F2.east) -- (S2.east);
\draw[gray,dashed] (F2.west) -- (S2.west);
\draw[gray,dashed] (F2.north) -- (S2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (S1.east) -- (T1.east);
\draw[gray,dashed] (S1.west) -- (T1.west);
\draw[gray,dashed] (S1.north) -- (T1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (S2.east) -- (T2.east);
\draw[gray,dashed] (S2.west) -- (T2.west);
\draw[gray,dashed] (S2.north) -- (T2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\draw[gray,dashed] (T1.east) -- (FF1.east);
\draw[gray,dashed] (T1.west) -- (FF1.west);
\draw[gray,dashed] (T1.north) -- (FF1.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\draw[gray,dashed] (T2.east) -- (FF2.east);
\draw[gray,dashed] (T2.west) -- (FF2.west);
\draw[gray,dashed] (T2.north) -- (FF2.north);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


}




%
%\node[draw,single arrow, orange,fill=orange!30] at (8,0.5,0) {GAP};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[circle,draw,blue,fill=blue!30] (A1) at (5,1,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,0.8,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\node[rectangle,draw,black,fill=orange!30]  (KL) at (6.85,-0.4,0) {KL Divergence};
\node[rectangle,draw,black,fill=orange!30]  (Loss) at (8,-0.4,0) {LDA Loss};
\draw[-latex] (KL) -- (Loss);
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer){};
\node[above of=A1, node distance=0.5cm] (hl) {$\mathbf{x}$};
\node[above of=B2, node distance=1.2cm] (hl) {$\mathbf{y}$};
\draw[gray,dashed] (PD1) -- (A3);
\draw[gray,dashed] (PU1) -- (A1);
\end{scope}

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);

\node[circle,draw,blue,fill=blue!30] (A1) at (5,-0.7,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,-0.9,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer) {};
\node[above of=A1, node distance=0.5cm] (hl) {$\mathbf{x}$};
\node[above of=B2, node distance=1.2cm] (hl) {$\mathbf{y}$};
\draw[gray,dashed] (PD2) -- (A3);
\draw[gray,dashed] (PU2) -- (A1);
\end{scope}


\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);







\end{tikzpicture}







% 
% \def\layersep{2.5cm}
% [shorten >=1pt,->,draw=black!50, node distance=\layersep]
%     \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%     \tikzstyle{neuron}=[circle,fill=black!25,minimum size=10pt,inner sep=0pt]
%     \tikzstyle{square-out}=[square,fill=black!25,minimum size=20pt,inner sep=0pt]
%     \tikzstyle{input neuron}=[neuron, fill=green!50];
%     \tikzstyle{output neuron}=[square-out, fill=red!50];
%     \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%     \tikzstyle{annot} = [text width=4em, text centered]
% 
%     % Draw the input layer nodes
%     \foreach \name / \y in {1,...,10}
%     % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%         \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};
% 
%     % Draw the hidden layer nodes
%     \foreach \name / \y in {1,...,3}
%         \path[yshift=0.5cm]
%             node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};
% 
%     % Draw the output layer node
%     \node[output neuron,pin={[pin edge={->}]right:LDA Loss} , right of=H-2] (O) {KL-distance};
% 
%     % Connect every node in the input layer with every node in the
%     % hidden layer.
%     \foreach \source in {1,...,10}
%         \foreach \dest in {1,...,3}
%             \path (I-\source) edge (H-\dest);
% 
%     % Connect every node in the hidden layer with the output layer
%     \foreach \source in {1,...,3}
%         \path (H-\source) edge (O) ;
% 
%     % Annotate the layers
%     \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
%     \node[annot,left of=hl] {Input layer};
%     \node[annot,right of=hl] {LDA projection};
% \end{tikzpicture}


==> abin_old.tex <==
%\documentclass[tikz,border=3.14pt]{standalone}
\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}

\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{
code={
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-right) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;

\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
 
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;

}
}}



% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}

\begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
font=\sffamily\small,scale=2]



\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.3,-\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 1}}] (\X - 0.2 ,0.9,0) -- (\X - 0.2, {2 + (-\Y)/2  - 2} ,0);
}
%%% For the input 1


\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.6,-4*\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 2}}] (\X - 0.5 ,-1.5,0) -- (\X - 0.5, -{2 + (-\Y)/2  - 2} ,0);
}
%%% For the input 2





\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X  - 0.3,-4*\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={CONV}}] (\X  ,-1.5,0) -- (\X  , -{2 + (-\Y)/2  - 2} ,0);
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X - 0.2,-4*\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X - 0.1,-4*\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);

}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X ,-\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={ conv}}] (\X + .05 ,0.5,0) -- (\X + .05 , -{2 + (-\Y)/2  - 2} ,0);

}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1,-\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
}

%For the blocks 1


%For blocks below%


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.2,-\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);

}




%
%\node[draw,single arrow, orange,fill=orange!30] at (8,0.5,0) {GAP};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[circle,draw,blue,fill=blue!30] (A1) at (5,1,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,0.8,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\node[rectangle,draw,black,fill=orange!30]  (KL) at (7,-0.4,0) {KL Distance};
\node[rectangle,draw,black,fill=orange!30]  (Loss) at (8,-0.4,0) {LDA Loss};
\draw[-latex] (KL) -- (Loss);
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer){};
\end{scope}

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);

\node[circle,draw,blue,fill=blue!30] (A1) at (5,-0.7,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,-0.9,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer) {};
\end{scope}


\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);



\end{tikzpicture}



% 
% \def\layersep{2.5cm}
% [shorten >=1pt,->,draw=black!50, node distance=\layersep]
%     \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%     \tikzstyle{neuron}=[circle,fill=black!25,minimum size=10pt,inner sep=0pt]
%     \tikzstyle{square-out}=[square,fill=black!25,minimum size=20pt,inner sep=0pt]
%     \tikzstyle{input neuron}=[neuron, fill=green!50];
%     \tikzstyle{output neuron}=[square-out, fill=red!50];
%     \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%     \tikzstyle{annot} = [text width=4em, text centered]
% 
%     % Draw the input layer nodes
%     \foreach \name / \y in {1,...,10}
%     % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%         \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};
% 
%     % Draw the hidden layer nodes
%     \foreach \name / \y in {1,...,3}
%         \path[yshift=0.5cm]
%             node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};
% 
%     % Draw the output layer node
%     \node[output neuron,pin={[pin edge={->}]right:LDA Loss} , right of=H-2] (O) {KL-distance};
% 
%     % Connect every node in the input layer with every node in the
%     % hidden layer.
%     \foreach \source in {1,...,10}
%         \foreach \dest in {1,...,3}
%             \path (I-\source) edge (H-\dest);
% 
%     % Connect every node in the hidden layer with the output layer
%     \foreach \source in {1,...,3}
%         \path (H-\source) edge (O) ;
% 
%     % Annotate the layers
%     \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
%     \node[annot,left of=hl] {Input layer};
%     \node[annot,right of=hl] {LDA projection};
% \end{tikzpicture}


==> abin_old__2_.tex <==

%
%

%

%



%\documentclass[tikz,border=3.14pt]{standalone}
\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}



	

\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{
code={
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-right) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;

\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
 
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;

}
}}



% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}

\begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
font=\sffamily\small,scale=2]



\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.4,-\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 1}}] (\X - 0.2 ,0.9,0) -- (\X - 0.2, {2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,0.4) (hl) {Anchor};
}


%%% For the input 1


\foreach \Y [count=\X] in {0.8}
{
\draw pic (box1-\X) at (\X - 0.5,-4*\Y,0) {fake box=white!70! green with dimensions 0 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={INPUT 2}}] (\X - 0.5 ,-1.5,0) -- (\X - 0.5, -{2 + (-\Y)/2  - 2} ,0);
\node at (-0.12,-2.4) (hl) {Negative};
}
%%% For the input 2





\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X  - 0,-4*\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={CONV}}] (\X  ,-1.5,0) -- (\X  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.45,1.65) (hl) {3x3 Kernel};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1 ,-4*\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.35,1.45) (hl) {3x3 Kernel};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X + 0.2 ,-4*\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (3.35,1.25) (hl) {3x3 Kernel};
\node at (4.35,-2.15) (hl) {3x3 Kernel};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X ,-\Y,0) {fake box=white!80!red with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={ conv}}] (\X + .05 ,0.5,0) -- (\X + .05 , -{2 + (-\Y)/2  - 2} ,0);
\node at (4.35,1.05) (hl) {3x3 Kernel};
\node at (3.25,-2.60) (hl) {3x3 Kernel};
}


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.1,-\Y,0) {fake box=white!70!blue with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={relu}}] (\X + .15 ,0.5,0) -- (\X + .25, -{2 + (-\Y)/2  - 2} ,0);
\node at (2.15,-3.00) (hl) {3x3 Kernel};
}

%For the blocks 1


%For blocks below%


\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
\draw pic (box1-\X) at (\X +0.2,-\Y,0) {fake box=white!30!gray with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%\path[black,decorate,decoration={text effects along path,text={pool}}] (\X + 0.25 ,0.5,0) -- (\X + 0.25  , -{2 + (-\Y)/2  - 2} ,0);
\node at (1.25,-3.35) (hl) {3x3 Kernel};
}




%
%\node[draw,single arrow, orange,fill=orange!30] at (8,0.5,0) {GAP};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[circle,draw,blue,fill=blue!30] (A1) at (5,1,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,0.8,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\node[rectangle,draw,black,fill=orange!30]  (KL) at (7,-0.4,0) {KL Distance};
\node[rectangle,draw,black,fill=orange!30]  (Loss) at (8,-0.4,0) {LDA Loss};
\draw[-latex] (KL) -- (Loss);
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer){};
\node[above of=A1, node distance=0.5cm] (hl) {512};
\node[above of=B2, node distance=1.2cm] (hl) {9};
\end{scope}

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);

\node[circle,draw,blue,fill=blue!30] (A1) at (5,-0.7,0) {~~~};
\node[circle,draw,blue,fill=blue!30,below=4pt of A1] (A2) {~~~};
\node[circle,draw,blue,fill=blue!30,below=35pt of A2] (A3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circle,draw,green,fill=green!40] (B1) at (6,-0.9,0) {~~~};
\node[circle,draw,green,fill=green!40,below=4pt of B1] (B2) {~~~};
\node[circle,draw,green,fill=green!40,below=10pt of B2] (B3) {~~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer) {};
\node[above of=A1, node distance=0.5cm] (hl) {512};
\node[above of=B2, node distance=1.2cm] (hl) {9};
\end{scope}


\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);











% 
% \def\layersep{2.5cm}
% [shorten >=1pt,->,draw=black!50, node distance=\layersep]
%     \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%     \tikzstyle{neuron}=[circle,fill=black!25,minimum size=10pt,inner sep=0pt]
%     \tikzstyle{square-out}=[square,fill=black!25,minimum size=20pt,inner sep=0pt]
%     \tikzstyle{input neuron}=[neuron, fill=green!50];
%     \tikzstyle{output neuron}=[square-out, fill=red!50];
%     \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%     \tikzstyle{annot} = [text width=4em, text centered]
% 
%     % Draw the input layer nodes
%     \foreach \name / \y in {1,...,10}
%     % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%         \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};
% 
%     % Draw the hidden layer nodes
%     \foreach \name / \y in {1,...,3}
%         \path[yshift=0.5cm]
%             node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};
% 
%     % Draw the output layer node
%     \node[output neuron,pin={[pin edge={->}]right:LDA Loss} , right of=H-2] (O) {KL-distance};
% 
%     % Connect every node in the input layer with every node in the
%     % hidden layer.
%     \foreach \source in {1,...,10}
%         \foreach \dest in {1,...,3}
%             \path (I-\source) edge (H-\dest);
% 
%     % Connect every node in the hidden layer with the output layer
%     \foreach \source in {1,...,3}
%         \path (H-\source) edge (O) ;
% 
%     % Annotate the layers
%     \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
%     \node[annot,left of=hl] {Input layer};
%     \node[annot,right of=hl] {LDA projection};
% \end{tikzpicture}


==> ient-defs-math.tex <==
%%-----------------------------------------------------------------------------
%% Standard-LaTeX-Dokument für Klausuren - Definitionen
%%-----------------------------------------------------------------------------
%% Autor:                                         M. Wien , v1,      11.01.2008
%%                                                C. Rohlfing, v1.1  25.04.2019
%%-----------------------------------------------------------------------------

% Spezielle Funktionen
\DeclareMathOperator{\erfc}{erfc}
\DeclareMathOperator{\lb}{lb}
\DeclareMathOperator{\rect}{rect}
\DeclareMathOperator{\sgn}{sgn}
\DeclareMathOperator{\si}{si}
\DeclareMathOperator{\Si}{Si}
\DeclareMathOperator{\sinc}{sinc}
\DeclareMathOperator{\prob}{Prob}
\DeclareMathOperator{\tr}{Tr}

% Differential, Real/Imaginaerteile, gerade/ungerade

%\newcommand{\dd}{\,\mathrm{d}}
\newcommand{\dd}{\mathop{}\!\mathrm{d}} %\mathop{} provides the thin space at the left when preceded by an ordinary symbol or a closing delimiter; the “d” after it inserts another thin space that's removed with \!


\newcommand{\A}{\mathrm{a}}
\newcommand{\D}{\mathrm{d}}
\newcommand{\G}{\mathrm{g}}
\newcommand{\J}{\mathrm{j}}
\newcommand{\U}{\mathrm{u}}
\newcommand{\E}{\mathrm{e}}
\newcommand{\OO}{\mathrm{o}}
\newcommand{\PP}{\mathrm{p}}

\let\Im\relax
\let\Re\relax
\DeclareMathOperator{\Im}{Im}
\DeclareMathOperator{\Re}{Re}

% Transformationen
\newcommand{\FT}{\mathcal{F}}
\newcommand{\IFT}{\mathcal{F}^{-1}}
\newcommand{\leftexp}[2]{{\vphantom{#2}}^{#1}{#2}}
%\newcommand{\trFT}{\stackrel{\FT}{\longleftrightarrow}}

% Doppelpfeil (Laplace, z)
\newcommand{\inTransform}[1]{\overset{{#1}}{\longleftrightarrow}}
\newcommand{\Transform}[1]{\overset{{#1}}{\longleftrightarrow}}
\newcommand{\inTransformH}[1]{\updownarrow {#1}}
\newcommand{\TransformH}[1]{\updownarrow {#1}}

% Transformations-Knochen, wie in der Doku vom trsym-Package
\newcommand{\tfh}{\TransformHoriz}
\newcommand{\itfh}{\InversTransformHoriz}
\newcommand{\tfv}{\TransformVert}
\newcommand{\itfv}{\InversTransformVert}

% Zahlenraeume
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Z}{\mathbb{Z}}

% Betrag, Norm
\providecommand{\abs}[1]{\left\lvert#1\right\rvert}
\providecommand{\norm}[1]{\left\lVert#1\right\rVert}


\newenvironment{nospaceflalign*}
 {\setlength{\abovedisplayskip}{0pt}\setlength{\belowdisplayskip}{0pt}%
  \csname flalign*\endcsname}
 {\csname endflalign*\endcsname\ignorespacesafterend}
 
\newenvironment{nospaceflalign}
 {\setlength{\abovedisplayskip}{0pt}\setlength{\belowdisplayskip}{0pt}%
  \csname flalign\endcsname}
 {\csname endflalign\endcsname\ignorespacesafterend}

==> rwth-colors.tex <==
% Define RWTH style colors

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% For HKS colors use the spotcolor package
% which predefines a number of such colors
% Main blue color is HKS 44 K
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% RGB colors used for screen
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% The main blue color, 100 and 50 are the
% most commonly used ones
% e.g. in the logo
\definecolor{rwth}   {RGB}{  0  84 159}
\definecolor{rwth-75}{RGB}{ 64 127 183}
\definecolor{rwth-50}{RGB}{142 186 229}
\definecolor{rwth-25}{RGB}{199 221 242}
\definecolor{rwth-10}{RGB}{232 241 250}

% All the other colors
% Secondary colors
\definecolor{black}   {RGB}{  0   0   0}
\definecolor{black-75}{RGB}{100 101 103}
\definecolor{black-50}{RGB}{156 158 159}
\definecolor{black-25}{RGB}{207 209 210}
\definecolor{black-10}{RGB}{236 237 237}

\definecolor{magenta}   {RGB}{227   0 102}
\definecolor{magenta-75}{RGB}{233  96 136}
\definecolor{magenta-50}{RGB}{241 158 177}
\definecolor{magenta-25}{RGB}{249 210 218}
\definecolor{magenta-10}{RGB}{253 238 240}

\definecolor{yellow}   {RGB}{255 237   0}
\definecolor{yellow-75}{RGB}{255 240  85}
\definecolor{yellow-50}{RGB}{255 245 155}
\definecolor{yellow-25}{RGB}{255 250 209}
\definecolor{yellow-10}{RGB}{255 253 238}

% The extended color spectrum
\definecolor{petrol}   {RGB}{  0  97 101}
\definecolor{petrol-75}{RGB}{ 45 127 131}
\definecolor{petrol-50}{RGB}{125 164 167}
\definecolor{petrol-25}{RGB}{191 208 209}
\definecolor{petrol-10}{RGB}{230 236 236}

\definecolor{turkis}   {RGB}{  0 152 161}
\definecolor{turkis-75}{RGB}{  0 177 183}
\definecolor{turkis-50}{RGB}{137 204 207}
\definecolor{turkis-25}{RGB}{202 231 231}
\definecolor{turkis-10}{RGB}{235 246 246}

\definecolor{grun}   {RGB}{ 87 171  39}
\definecolor{grun-75}{RGB}{141 192  96}
\definecolor{grun-50}{RGB}{184 214 152}
\definecolor{grun-25}{RGB}{221 235 206}
\definecolor{grun-10}{RGB}{242 247 236}

\definecolor{maigrun}   {RGB}{189 205   0}
\definecolor{maigrun-75}{RGB}{208 217  92}
\definecolor{maigrun-50}{RGB}{224 230 154}
\definecolor{maigrun-25}{RGB}{240 243 208}
\definecolor{maigrun-10}{RGB}{249 250 237}

\definecolor{orange}   {RGB}{246 168   0}
\definecolor{orange-75}{RGB}{250 190  80}
\definecolor{orange-50}{RGB}{253 212 143}
\definecolor{orange-25}{RGB}{254 234 201}
\definecolor{orange-10}{RGB}{255 247 234}

\definecolor{rot}   {RGB}{204   7  30}
\definecolor{rot-75}{RGB}{216  92  65}
\definecolor{rot-50}{RGB}{230 150 121}
\definecolor{rot-25}{RGB}{243 205 187}
\definecolor{rot-10}{RGB}{250 235 227}

\definecolor{bordeaux}   {RGB}{161  16  53}
\definecolor{bordeaux-75}{RGB}{182  82  86}
\definecolor{bordeaux-50}{RGB}{205 139 135}
\definecolor{bordeaux-25}{RGB}{229 197 192}
\definecolor{bordeaux-10}{RGB}{245 232 229}

\definecolor{violett}   {RGB}{ 97  33  88}
\definecolor{violett-75}{RGB}{131  78 117}
\definecolor{violett-50}{RGB}{168 133 158}
\definecolor{violett-25}{RGB}{210 192 205}
\definecolor{violett-10}{RGB}{237 229 234}

\definecolor{lila}   {RGB}{122 111 172}
\definecolor{lila-75}{RGB}{155 145 193}
\definecolor{lila-50}{RGB}{188 181 215}
\definecolor{lila-25}{RGB}{222 218 235}
\definecolor{lila-10}{RGB}{242 240 247}


==> snn.tex <==
\usetikzlibrary{arrows,decorations.pathmorphing,backgrounds,positioning,fit,petri, decorations.pathreplacing,shadows,calc}

%\documentclass[tikz,border=3.14pt]{standalone}
%\usetikzlibrary{3d,decorations.text,shapes.arrows,positioning,fit,backgrounds}

\tikzset{pics/fake box/.style args={% #1=color, #2=x dimension, #3=y dimension, #4=z dimension
#1 with dimensions #2 and #3 and #4}{%
code={%
\draw[gray,ultra thin,fill=#1]  (0,0,0) coordinate(-front-bottom-left) to
++ (0,#3,0) coordinate(-front-top-left) --++
(#2,0,0) coordinate(-front-top-right) --++ (0,-#3,0) 
coordinate(-front-bottom-right) -- cycle;

\draw[gray,ultra thin,fill=#1] (0,#3,0)  --++ 
 (0,0,#4) coordinate(-back-top-left) --++ (#2,0,0) 
 coordinate(-back-top-right) --++ (0,0,-#4)  -- cycle;
 
\draw[gray,ultra thin,fill=#1!80!black] (#2,0,0) --++ (0,0,#4) coordinate(-back-bottom-right)
--++ (0,#3,0) --++ (0,0,-#4) -- cycle;
}
}}

\tikzset{pics/flat box/.style args={% #1=color, #2=y dimension, #3=z dimension,
#1 with dimensions #2 and #3}{%
code={%
\draw[gray,ultra thin,fill=#1] (0,0,0) coordinate(-front-bottom) --++ (0,0,#3) coordinate(-back-bottom)
--++ (0,#2,0) coordinate(-back-top) --++ (0,0,-#3)  coordinate(-front-top) -- cycle;
}
}}

\tikzset{pics/dash box/.style args={% #1=color, #2=y dimension, #3=z dimension
#1 with dimensions #2 and #3}{%
code={%
 
\draw[dashed,#1,thick] (0,0,0) coordinate(-c1) --++ (0,0,#3) coordinate(-c2)
--++ (0,#2,0) coordinate(-c3) --++ (0,0,-#3)  coordinate(-c4) -- cycle;
}
}}

% from https://tex.stackexchange.com/a/52856/121799
\tikzset{circle dotted/.style={dash pattern=on .05mm off 2mm,
                                         line cap=round}}

\tikzstyle{circblue} = [circle,draw,rwth,fill=rwth-50]%%\tikzstyle{circblue} = [circle,draw,blue,fill=blue!30]%
\tikzstyle{circgreen} = [circle,draw,grun,fill=grun-50]%%\tikzstyle{circgreen} = [circle,draw,green,fill=green!40]%


\begin{tikzpicture}[x={(1,0)},y={(0,1)},z={({cos(60)},{sin(60)})},
font=\sffamily\small,scale=2]



%%%%%% BOTTOM BRANCH

%%% Image 2
% \foreach \Y [count=\X] in {0.8}
% {
%   \draw pic (img2) at (\X - 0.5,-4*\Y,0) {flat box=grun-50 with dimensions {4*\Y} and 2*\Y} ;
%   \draw pic (dbox-img2) at (\X-0.5,-2.5*\Y,0.25*\Y) {dash box=black with dimensions {0.5*\Y} and 0.5*\Y} ;
% }
% \node[grun-75,anchor=east] at ($(img2-front-bottom)!0.5!(img2-front-top)+(-0.25,0)$) {Img. 2};
% 
% \foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
% {
%   \draw pic (box-red-\X) at (\X  - 0,-4*\Y,0) {fake box=rot-25 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
% }
% 
% \foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
% {
%   \draw pic (box-blue-\X) at (\X +0.1 ,-4*\Y,0) {fake box=lila-50 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
% }
% 
% \foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
% {
%   \draw pic (box-gray-\X) at (\X + 0.2 ,-4*\Y,0) {fake box=black-50 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
%   \draw pic (dbox-\X) at (\X+0.2+0.125,-2.5*\Y,0.25*\Y) {dash box=black with dimensions {0.5*\Y} and 0.5*\Y};
% }

%% Connections between dboxes
% \begin{scope}
%   %\draw[thick,red] (box-red-1-front-bottom-left) -- (img2-front-bottom) -- (img2-front-top)  -- (img2-back-top) --  (box-red-1-back-top-left) -- (box-red-1-front-top-left) -- cycle;
%   \clip (box-red-1-front-bottom-left) -- (img2-front-bottom) -- (img2-front-top)  -- (img2-back-top) --  (box-red-1-back-top-left) -- (box-red-1-front-top-left) -- cycle;
%   \foreach \c in {1,...,4}
%   {
%     \draw[black-75,dashed](dbox-img2-c\c) -- (dbox-1-c\c);
%   }
% \end{scope}
% 
% \foreach \i/\j in {1/2,2/3,3/4}
% {
% \begin{scope}
%   %\draw[thick,red] (box-red-\j-front-bottom-left) -- (box-gray-\i-front-bottom-right) -- (box-gray-\i-front-top-right)  -- (box-gray-\i-back-top-right) --  (box-red-\j-back-top-left) -- (box-red-\j-front-top-left) -- cycle;
%   \clip (box-red-\j-front-bottom-left) -- (box-gray-\i-front-bottom-right) -- (box-gray-\i-front-top-right)  -- (box-gray-\i-back-top-right) --  (box-red-\j-back-top-left) -- (box-red-\j-front-top-left) -- cycle;
%   \foreach \c in {1,...,4}
%   {
%     \draw[black-75,dashed](dbox-\i-c\c) -- (dbox-\j-c\c);
%   }
% \end{scope}
% }


%%%% TOP BRANCH

%%% Image 1
\foreach \Y [count=\X] in {0.8}
{
  \draw pic (img1) at (\X - 0.5,-\Y,0) {flat box=grun-50 with dimensions {4*\Y} and 2*\Y} ;
  \draw pic (dbox-img1) at (\X-0.5,0.5*\Y,0.25*\Y) {dash box=black with dimensions {0.5*\Y} and 0.5*\Y} ;
}
\node[grun-75,anchor=east] at ($(img1-front-bottom)!0.5!(img1-front-top)+(-0.25,0)$) {Img. 1};

\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
  \draw pic (bbox-red-\X) at (\X ,-\Y,0) {fake box=rot-25 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
}

\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
  \draw pic (bbox-blue-\X) at (\X +0.1,-\Y,0) {fake box=lila-50 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
}

\foreach \Y [count=\X] in {0.8,0.7,0.6,0.5}
{
  \draw pic (bbox-gray-\X) at (\X +0.2,-\Y,0) {fake box=black-50 with dimensions 0.25 and {4*\Y} and 2*\Y} ;
  \draw pic (dbox-\X) at (\X+0.2+0.125,0.5*\Y,0.25*\Y) {dash box=black with dimensions {0.5*\Y} and 0.5*\Y};
}
%% Connections between dboxes
\begin{scope}
  %\draw[thick,red] (box-red-1-front-bottom-left) -- (img2-front-bottom) -- (img2-front-top)  -- (img2-back-top) --  (box-red-1-back-top-left) -- (box-red-1-front-top-left) -- cycle;
  \clip (bbox-red-1-front-bottom-left) -- (img1-front-bottom) -- (img1-front-top)  -- (img1-back-top) --  (bbox-red-1-back-top-left) -- (bbox-red-1-front-top-left) -- cycle;
  \foreach \c in {1,...,4}
  {
    \draw[black-75,dashed](dbox-img1-c\c) -- (dbox-1-c\c);
  }
\end{scope}

\foreach \i/\j in {1/2,2/3,3/4}
{
\begin{scope}
  %\draw[thick,red] (box-red-\j-front-bottom-left) -- (box-gray-\i-front-bottom-right) -- (box-gray-\i-front-top-right)  -- (box-gray-\i-back-top-right) --  (box-red-\j-back-top-left) -- (box-red-\j-front-top-left) -- cycle;
  \clip (bbox-red-\j-front-bottom-left) -- (bbox-gray-\i-front-bottom-right) -- (bbox-gray-\i-front-top-right)  -- (bbox-gray-\i-back-top-right) --  (bbox-red-\j-back-top-left) -- (bbox-red-\j-front-top-left) -- cycle;
  \foreach \c in {1,...,4}
  {
    \draw[black-75,dashed](dbox-\i-c\c) -- (dbox-\j-c\c);
  }
\end{scope}
}



%
%\node[draw,single arrow, orange,fill=orange!30] at (8,0.5,0) {GAP};
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\node[circblue] (A1) at (5,1,0) {~~};
\node[circblue,below=4pt of A1] (A2) {~~};
\node[circblue,below=35pt of A2] (A3) {~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circgreen] (B1) at (6,0.8,0) {~~};
\node[circgreen,below=4pt of B1] (B2) {~~};
\node[circgreen,below=10pt of B2] (B3) {~~};
\node[rectangle,draw,black,fill=orange-25]  (KL) at (6.85,-0.4,0) {KL Divergence};
\node[rectangle,draw,black,fill=orange-25]  (Loss) at (8,-0.4,0) {LDA Loss};
\draw[-latex] (KL) -- (Loss);
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer){};
\node[above of=A1, node distance=0.5cm] (hl) {$\mathbf{x}$};
\node[above of=B2, node distance=1.2cm] (hl) {$\mathbf{y}$};
%\draw[gray,dashed] (PD1) -- (A3);
%\draw[gray,dashed] (PU1) -- (A1);
\end{scope}
\draw[black-75,dashed] ($(bbox-gray-4-front-bottom-right)!0.5!(bbox-gray-4-back-bottom-right)$) -- (A3);
\draw[black-75,dashed] ($(bbox-gray-4-front-top-right)!0.5!(bbox-gray-4-back-top-right)$) -- (A1);

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);

\node[circblue] (A1) at (5,-0.7,0) {~~};
\node[circblue,below=4pt of A1] (A2) {~~};
\node[circblue,below=35pt of A2] (A3) {~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (A2) -- (A3);
\node[circgreen] (B1) at (6,-0.9,0) {~~};
\node[circgreen,below=4pt of B1] (B2) {~~};
\node[circgreen,below=10pt of B2] (B3) {~~};
\draw[circle dotted, line width=2pt,shorten <=2pt] (B2) -- (B3);
\begin{scope}[on background layer]
\node[orange,thick,rounded corners,fill=orange!30,fit=(A1) (A3)]{};
\node[orange,thick,rounded corners,fill=orange!30,fit=(B1) (B3)] (LDA-layer) {};
\node[above of=A1, node distance=0.5cm] (hl) {$\mathbf{x}$};
\node[above of=B2, node distance=1.2cm] (hl) {$\mathbf{y}$};
%\draw[gray,dashed] (PD2) -- (A3);
%\draw[gray,dashed] (PU2) -- (A1);
\end{scope}
\draw[black-75,dashed] ($(box-gray-4-front-bottom-right)!0.5!(box-gray-4-back-bottom-right)$) -- (A3);
\draw[black-75,dashed] ($(box-gray-4-front-top-right)!0.5!(box-gray-4-back-top-right)$) -- (A1);

\foreach \Y in {1,2,3}
\foreach \X in {1,2,3}
{\draw[-latex] (A\X) -- (B\Y);}
\draw[-latex] (LDA-layer) -- (KL);



\end{tikzpicture}







% 
% \def\layersep{2.5cm}
% [shorten >=1pt,->,draw=black!50, node distance=\layersep]
%     \tikzstyle{every pin edge}=[<-,shorten <=1pt]
%     \tikzstyle{neuron}=[circle,fill=black!25,minimum size=10pt,inner sep=0pt]
%     \tikzstyle{square-out}=[square,fill=black!25,minimum size=20pt,inner sep=0pt]
%     \tikzstyle{input neuron}=[neuron, fill=green!50];
%     \tikzstyle{output neuron}=[square-out, fill=red!50];
%     \tikzstyle{hidden neuron}=[neuron, fill=blue!50];
%     \tikzstyle{annot} = [text width=4em, text centered]
% 
%     % Draw the input layer nodes
%     \foreach \name / \y in {1,...,10}
%     % This is the same as writing \foreach \name / \y in {1/1,2/2,3/3,4/4}
%         \node[input neuron, pin=left:Input \#\y] (I-\name) at (0,-\y) {};
% 
%     % Draw the hidden layer nodes
%     \foreach \name / \y in {1,...,3}
%         \path[yshift=0.5cm]
%             node[hidden neuron] (H-\name) at (\layersep,-\y cm) {};
% 
%     % Draw the output layer node
%     \node[output neuron,pin={[pin edge={->}]right:LDA Loss} , right of=H-2] (O) {KL-distance};
% 
%     % Connect every node in the input layer with every node in the
%     % hidden layer.
%     \foreach \source in {1,...,10}
%         \foreach \dest in {1,...,3}
%             \path (I-\source) edge (H-\dest);
% 
%     % Connect every node in the hidden layer with the output layer
%     \foreach \source in {1,...,3}
%         \path (H-\source) edge (O) ;
% 
%     % Annotate the layers
%     \node[annot,above of=H-1, node distance=1cm] (hl) {Hidden layer};
%     \node[annot,left of=hl] {Input layer};
%     \node[annot,right of=hl] {LDA projection};
% \end{tikzpicture}

